Moving Participants Turtle Consensus

We present Moving Participants Turtle Consensus (MPTC), an asynchronous consensus protocol for crash and Byzantine-tolerant distributed systems. MPTC uses various moving target defense strategies to tolerate certain Denial-of-Service (DoS) attacks issued by an adversary capable of compromising a bounded portion of the system. MPTC supports on the fly reconfiguration of the consensus strategy as well as of the processes executing this strategy when solving the problem of agreement. It uses existing cryptographic techniques to ensure that reconfiguration takes place in an unpredictable fashion thus eliminating the adversary's advantage on predicting protocol and execution-specific information that can be used against the protocol. We implement MPTC as well as a State Machine Replication protocol and evaluate our design under different attack scenarios. Our evaluation shows that MPTC approximates best case scenario performance even under a well-coordinated DoS attack.

==> byzantine_correctness.tex <==
\section{Byzantine MPTC Correctness discussion}
\label{asec:byz_correct}

The byzantine version of MPTC must satisfy the properties described above as 
well as robustness and unpredictability. We again assume a valid $\mcp$ 
containing correct BFT protocols, MPTC execution under $\mca_\mcp$ as well as a 
set of configurations $\mcc$ such that a conforming interleaving exists. The 
arguments for all of these properties are similar to those in 
Section~\ref{ssec:mptc_proofs}. In fact, the termination arguments for the 
byzantine MPTC are exactly the same. Robustness and unpredictability are also 
exactly the same and our arguments are mainly borrowed from the corresponding 
arguments of the byzantine agreement protocol of~\cite{Cachin05}. For the rest 
of the properties we have the following results:

\begin{lemma}
\label{lem:byz_mptc_validity}
Byzantine MPTC satisfies validity.
\end{lemma}

\begin{proof}
By correctness of the underlying BFT, any decision made by an honest process 
during Phase 1 respects validity. A decision during Phase 3 can only 
occur if at least $f+1$ processes send the same decision outcome $(D, v)$ for 
some $v \in \mcv$. For that to happen at least one honest process must have 
computed that outcome during Phase 1. Thus that value must have been proposed 
by some process.
%It holds trivially due to the fact that the first decision by an honest process is done during Phase 2 and by validity of the BFT run during that round it must have been proposed.
\end{proof}

\begin{lemma}
\label{lem:byz_mptc_agreement}
Byzantine MPTC satisfies agreement.
\end{lemma}

\begin{proof}
Note that Phase 1 respects agreement by the correctness of the protocols in 
$\mcp$. Observe that honest processes can only decide during Phase 3 if 
at least $f+1$ processes have decided the same value. This means that if an 
honest process decides $v$ during Phase 3 of MPTC at least one honest 
process has already decided $v$. Using similar arguments to those in 
Lemma~\ref{correctness:agreement}, we can show that at any point during MPTC 
execution any two honest processes that decide must decide the same value.
\end{proof}

\begin{lemma}
\label{lem:byz_mptc_unanimity}
Byzantine MPTC satisfies unanimity.
\end{lemma}

\begin{proof}
Assume that all honest processes are initialized with the same value $v \in 
\mcv$. Since the BFT protocols in $\mcp$ are correct, honest processes getting 
into Phase 1 with the same value, $v$, can only compute outcomes $(D, v)$, $(M, 
v)$ and $(U, v)$. Otherwise it would mean that honest processes can change 
their proposals between rounds of the BFT protocol in question (e.g., via the 
influence of the faulty processes) and eventually decide a different value, 
which would violate unanimity of the BFT protocol. Therefore, at the end of 
Phase 1 all honest processes will end up with outcomes containing $v$. $v$ will 
be the most frequent value in any subset of $\mcp_f - f$ outcomes since $\mcp_f 
\geq 3f + 1$ and at least $2f+1$ processes are correct. As a result Phases 2 
and 3 will have all honest processes updating their outcomes and proposals to 
$v$. Consequently, all honest processes will eventually move to subsequent 
rounds with $v$ as their proposal and thus $v$ will be the only value that can 
be decided by some honest process.
\end{proof}

==> discussion.tex <==
\section{Discussion}\label{sec:mptc_discussion}

%The Turtle Consensus construction shows that we can dynamically change between consensus protocols across rounds on the fly.
%More interestingly, it showcases a configuration element on which diversity can be introduced to increase the system's resistance against attacks.
%
%Regular reconfiguration of the protocol run in each round or set of rounds can help avoid protocol specific exploits and pathogenic crashes that can dramatically degrade the performance of the protocol under execution.
%A faulty leader in a leader-oriented consensus protocol, e.g. Paxos~\cite{Lamport98}, can easily stall the protocol's progress while a faulty process in a Ben-OR instance has less influence in the number of rounds it takes the protocol to reach a decision.
%Such transitions can cause uncertainty to attackers that rely on crashing or saturating the right targets during the protocols' execution.
%A very interesting question that we consider future work is how to select the next consensus protocol to run, how often and the preconditions for a reconfiguration to take place.
%We consider that bookkeeping of execution information including but not limited to, unnatural message rates, occurrences of slow-paths or timeouts and culprit processes behind such behaviors, can provide adaptive strategies for protocol selection.
%%A simple example switching strategy can be for processes to monitor the number of rounds it takes before they make a decision and if that number surpasses a threshold they move to a different protocol.
%
%The selection strategy however is itself a protocol and thus susceptible to attacks.
%Imagine the case where at any given round a leader process is elected which selects and informs the rest of the processes about the protocol they should run in the current round.
%Such an approach would be relatively fast. 
%A leader can be elected in one step by observing the current round number, and then the other processes can learn the protocol in half a round-trip time.
%The introduction of a leader however also introduces a new target for attack.
%An attacker knowing who the leader is can issue a DOS attack at it and keep the rest of the processes waiting for a configuration message.
%In addition, this type of attack could be persisted in multiple rounds if the attacker knows the leader election procedure.
%We can easily fix such targeted attacks by having the processes decide the protocol solely according to the round number.
%An informed attacker knowing the round number and the mapping between round and protocols can still devise and launch separate attacks on each round but at least in that case the vulnerabilities are limited only to those of each protocol.
%More elaborate procedures for protocol selection may become necessary depending on the knowledge of the attacker.
%However, one should be aware of the trade-off between performance and attack-tolerance that comes with such configuration selection techniques.
%
%In this work, the configuration of the system is focused entirely on the protocol to be run on each round.
%There are other elements that we can diversify to improve the robustness of the system.
%One such element is having only a subset of the processes run the selected protocol.
%Provided that $|N|$ is sufficiently large we could, during the configuration selection, choose a sufficiently large subset of $N$ on which the protocol in the configuration may run.
%This further obfuscates the attack surface of the system to outside and potentially inside attackers.
%We consider this configuration extension as direction for future work.
%
%%A non faulty leader will choose a quorum of processes that execute a round of a consensus protocol.
%%Note that if $|N| = 3t + 1$ the quorum will consist of the entire set of processes since we are interested in protocols that can handle Byzantine failures.
%%This does not offer any advantages in obfuscating the configuration from Byzantine processes.
%%A better bound for the number of processes in the system is $|N| \geq 4t + 1$ which creates an uncertainty on each process regarding the quorum members since only those processes are informed regarding membership.
%%This uncertainty can prevent Byzantine processes from interfering with the actual consensus protocol execution if such processes are not part of the quorum.
%%This condition however can be difficult to satisfy.
%%If a Byzantine process is in the quorum, it can easily notify others of the quorum members' identities as well as of the protocol they run and thus organize a DOS or a protocol dependent attack with the rest of the quorum.
%%By simply choosing a quorum uniformly at random the probability of a Byzantine being a part of the protocol is far from negligible for realistic sizes of $N$.
%%Entire exclusion of Byzantine processes is not necessary, however, to benefit from selecting a ``private'' quorum.
%%Messages originating from processes outside a quorum can be safely ignored during the execution of the protocol selected thus limiting the resources that an adversary has to issue attacks on the quorum even if it has complete information of the quorum membership.
%%In addition, misbehaving processes might be exposed to correct processes in the quorum which can then be used to make better informed decisions on future quorum selections.
%
%%Similarly, regularly selecting a different protocol can help avoid protocol specific exploits that can dramatically degrade the performance of the protocol under execution.
%%A faulty leader in a leader-oriented consensus protocol, e.g. PBFT~\cite{CL99}, can easily stall the protocol while a faulty process in a Ben-OR instance has less influence in the number of rounds it takes the protocol to reach a decision.
%%As in the case of the quorum selection, bookkeeping of execution information including but not limited to, invalid messages, unnatural message rates, occurrences of slow-path and culprit processes behind such behaviors, can provide adaptive strategies for protocol selection.
